Pixel-wise Dense Detector for Image Inpainting

Recent GAN-based image inpainting approaches adopt an average strategy to discriminate the generated image and output a scalar, which inevitably lose the position information of visual artifacts. Moreover, the adversarial loss and reconstruction loss (e.g., l1 loss) are combined with tradeoff weights, which are also difficult to tune. In this paper, we propose a novel detection-based generative framework for image inpainting, which adopts the min-max strategy in an adversarial process. The generator follows an encoder-decoder architecture to fill the missing regions, and the detector using weakly supervised learning localizes the position of artifacts in a pixel-wise manner. Such position information makes the generator pay attention to artifacts and further enhance them. More importantly, we explicitly insert the output of the detector into the reconstruction loss with a weighting criterion, which balances the weight of the adversarial loss and reconstruction loss automatically rather than manual operation. Experiments on multiple public datasets show the superior performance of the proposed framework. The source code is available at https://github.com/Evergrow/GDN_Inpainting.

==> EGauthorGuidelines-body_with_teaser_old.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.03, Dec 14, 2018


\title[Pixel-wise Dense Detector for Image Inpainting]%
      {Pixel-wise Dense Detector for Image Inpainting}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[R.Zhang et al.]
{\parbox{\textwidth}{\centering 
        Ruisong Zhang$^{1,2}$\orcid{0000-0002-7051-3309}, 
        Weize Quan$^{1,2}$\orcid{0000-0003-0892-581X}, 
        Baoyuan Wu$^{3,4}$\orcid{0000-0003-2183-5990}, 
        Zhifeng Li$^5$ %\orcid{0000-0001-7756-0901}
        and Dong-Ming Yan$^{1,2}$\thanks{Corresponding Author}\orcid{0000-0003-2209-2404}
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$National Laboratory of Pattern Recognition, Institute of Automation, Chinese Academy of Sciences, Beijing 100190, China\\
         $^2$School of Artificial Intelligence, University of Chinese Academy of Sciences, Beijing 100049, China \\
         $^3$School of Data Science, the Chinese University of Hong Kong, Shenzhen, China\\
         $^4$Secure Computing Lab of Big Data, Shenzhen Research Institute of Big Data, China\\
         $^5$Tencent AI Lab, Shenzhen, China
%        $^2$ Another Department to illustrate the use in papers from authors
%             with different affiliations
       }
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

\teaser{
    \centering
    \includegraphics[width=0.95\textwidth]{Teaser.pdf}
    \caption{Image inpainting results by our proposed method.}
    \label{Fig:Intro}
}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract}
   Recent GAN-based image inpainting approaches adopt an average strategy to discriminate the generated image and output a scalar, which inevitably lose the position information of visual artifacts. Moreover, the adversarial loss and reconstruction loss (\textit{e.g.}, $\ell_1$ loss) are combined with tradeoff weights, which are also difficult to tune. In this paper, we propose a novel detection-based generative framework for image inpainting, which adopts the min-max strategy in an adversarial process. The generator follows an encoder-decoder architecture to fill the missing regions, and the detector using weakly supervised learning localizes the position of artifacts in a pixel-wise manner. Such position information makes the generator pay attention to artifacts and further enhance them. More importantly, we explicitly insert the output of the detector into the reconstruction loss with a weighting criterion, which balances the weight of the adversarial loss and reconstruction loss automatically rather than manual operation. Experiments on multiple public datasets show the superior performance of the proposed framework. The source code is available at \url{https://github.com/Evergrow/GDN\_Inpainting}.
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see https://www.acm.org/publications/computing-classification-system/1998)
% \begin{classification} % according to https://www.acm.org/publications/computing-classification-system/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
%   (see https://www.acm.org/publications/class-2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010382.10010383</concept_id>
<concept_desc>Computing methodologies~Image processing</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Image processing}


\printccsdesc   
\end{abstract}  
%-------------------------------------------------------------------------
\input{ch1-introduction}
\input{ch2-relatedwork}
\input{ch3-method}
\input{ch4-experiment}
\input{ch5-conclusion}

%-------------------------------------------------------------------------
% bibtex
%\bibliographystyle{eg-alpha}
%\bibliography{egbibsample}        

% biblatex with biber
\printbibliography                

%-------------------------------------------------------------------------


\end{document}

